Cell behavior in the face of uncertainty

Organisms that grow and survive in uncertain environments may need to change their physiological state as the environment changes. When the environment is uncertain, one strategy known as bet-hedging is to make these changes randomly and independently of the environment, to ensure that at least part of the population is well adapted. Organisms that collect information from their environment may also use this information to modulate their changes of physiological states. We review these different strategies and point out parallels with the theory of optimal financial investments.

==> ECPC book - Part V - UNC/backup_08_10_22/macros-old.tex <==
% This is the central macro collection file that is used to define
% LaTeX macros for the final compiled book
%
% DO NOT APPLY ANY CHANGES TO THIS FILE UNLESS THIS WAS APPROVED BY THE BOOK EDITORS!
%
% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
%\usepackage[USenglish]{babel}
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{float}
\usepackage{geometry}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{lmodern}
\usepackage{mdframed}
\usepackage[numbers]{natbib}
\usepackage{siunitx}%
\usepackage{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MACROS ADDED on April 16th
%
% general %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[textsize=footnotesize,textwidth=2.8cm]{todonotes}
\usepackage[version=4]{mhchem}
%
% for chapter MET %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage[colorlinks=true, linkcolor=blue, urlcolor=blue]{hyperref}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\red[1]{\textcolor{red}{#1}}
%
% for chapter CBM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{physics}
\newcommand{\ve}[1]{\mathvectorfont{#1}}
\newcommand{\mat}[1]{\mathmatrixfont{#1}}
%
% for chapter SMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathtools}
%
% for chapter UNC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\s}{\sigma}
\renewcommand{\L}{\Lambda}
\newcommand{\dkl}{D_{\text{KL}}}
\newcommand{\Wxi}{\mathcal{W}_{x_i}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\lp}{\log\!\text{-}\mathrm{cap}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\R}{\mathrm{r}}
\newcommand{\B}{\mathrm{b}}
\newcommand{\odds}{\mathrm{o}}
\newcommand{\diff}{\mathrm{d}}
\renewcommand{\underline}[1]{\mathbf{#1}}
\newcommand{\intsimpldetail}[2]{\int_{\mathbb{R}^M_+}\diff \mathbf{b} ~ \delta \left( \sum_{\tilde{x}} \B_{\tilde{x}} - #1 \right) ~ #2}
\newcommand{\intsimpl}[1]{\int_{\mathcal{B}} \diff \mathbf{b} ~ #1}
\newcommand{\N}{\noindent}
%
%
% for chapter PAT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Esc}{E}
\newcommand{\activity}{A}
\newcommand{\fluxcost}{a}
\newcommand{\hminus}{h}
\newcommand{\vPW}{v_{\rm pw}}
\newcommand{\enzymev}{\mathbf{e}}
\newcommand{\rrl}{\fluxcost_{v_l}}
\newcommand{\rrlmin}{\rrl^{\rm cat}}
\newcommand{\metbene}{b^{\rm (c)}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\concS}{s}
\newcommand{\concP}{p}
\newcommand{\e}{\mathrm{e}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\ratelaw}{f}
\definecolor{c1}{rgb}{0,0,0.8}
\definecolor{c2}{rgb}{0.25,0.,0.6}
\definecolor{c3}{rgb}{0.6,0.,0.3} 
\definecolor{c4}{rgb}{1,0,0}
\definecolor{c5}{rgb}{.5,0.2,0}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
% PROJECT SPECIFIC MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includechapterauthors}[1]{%
\par\noindent%
\textbf{Written by} #1\\[-3ex]%
}%

\newcommand{\chapteracknowledgments}[1]{
\par\noindent%
\textbf{Contributions:} #1\\[-3ex]%
}

\newcommand{\chapterkeywords}[1]{%
\par\noindent%
\textbf{Keywords:} #1\\[-3ex]%
}%

\newcommand{\comment}[1]{{\color{red}#1}}

\newcommand{\chapterroot}{./chapters/TEMPLATE/}% This refers to chapter directory

\newcommand{\copyrightinfo}[1]%{}
  {{\color{magenta}\textsc{Copyright Info:} #1}}

%
% Math macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Real}{\mathbb{R}} % real numbers
\newcommand{\Natu}{\mathbb{N}} % natural numbers
\newcommand{\Inte}{\mathbb{Z}} % integers
%
\newcommand{\expe}{\mathrm{e}}% Euler s number
\newcommand{\imagi}{\mathrm{i}}% imaginary unit
\newcommand{\intd}{\mathrm{d}}% differential-d
%
\newcommand{\mathvectorfont}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mathmatrixfont}[1]{\mathbf{#1}}
%
\newcommand{\avec}{\mathvectorfont{a}}
\newcommand{\varphivec}{\mathvectorfont{\varphi}}
%
\newcommand{\Amat}{\mathmatrixfont{A}}

%
% Metabolic modeling macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\kcat}{k_{\rm cat}}
\newcommand{\kcati}{k_{\rm cat,i}}
\newcommand{\kcatl}{k_{{\rm cat},l}}
\newcommand{\kcatplus}{k_{\rm cat}^+}
\newcommand{\kcatplusl}{k_{{\rm cat},l}^+}
\newcommand{\kcatminus}{k_{\rm cat}^-}
\newcommand{\km}{K_{{\rm M}}}
\newcommand{\kmS}{K_{{\rm S}}}
\newcommand{\kmP}{K_{{\rm P}}}
\newcommand{\Keq}{K_{\rm eq}} % equilibrium constant

% BOXES :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% To make use of
% (a) (future) key-value extensions,
% (b) numbering,
% (c) referencing and
% (d) mdframed boxes,
% we use the following "hack":
% (i) use mdframed for the definition of the boxes
% (ii) wrap them in "classically defined" environments that take care of labels, titles etc.
%
% MAYBE: - easier handling/cleaner code when using "startcode" and "endcode" from the mdframed package?
%  - "derive" everything from one "numbered box" code?
%  - change numbering (e.g. all boxes together)?
%
\makeatletter
% CHAPTER HIGHLIGHTS BOX %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newmdenv[linecolor=blue!50!black,
frametitlerule=true,
frametitle={Chapter highlights},
frametitlebackgroundcolor=blue!10%,
]{chapterhighlights}

% ECONOMIC ANALOGY BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@ecoanaTitle}{}%
\define@key{EPCPecoana}{label}{\label{#1}}%
\define@key{EPCPecoana}{title}{\renewcommand{\EPCP@ecoanaTitle}{(\textsl{#1})}}%
\newcounter{ecoanaboxcounter}\setcounter{ecoanaboxcounter}{0}%
\renewcommand{\theecoanaboxcounter}{\arabic{chapter}.\arabic{section}.\alph{ecoanaboxcounter}}%
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitlebackgroundcolor=blue!10]{Ecoblock-pre}
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitle={Economic analogy},frametitlebackgroundcolor=blue!10]{Ecoblock*}
\newenvironment{Ecoblock}[1][]{\begin{Ecoblock-pre}%
  [frametitle={Economic analogy \refstepcounter{ecoanaboxcounter}\setkeys{EPCPecoana}{#1}\theecoanaboxcounter{} \EPCP@ecoanaTitle}%
  \renewcommand{\EPCP@ecoanaTitle}{}%
  ]}{\end{Ecoblock-pre}}%

% Philosophcal question BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@philquestTitle}{}%
\define@key{EPCPphilquest}{label}{\label{#1}}%
\define@key{EPCPphilquest}{title}{\renewcommand{\EPCP@philquestTitle}{(\textsl{#1})}}%
\newcounter{philquestboxcounter}\setcounter{philquestboxcounter}{0}%
\renewcommand{\thephilquestboxcounter}{\arabic{chapter}.\arabic{section}.\alph{philquestboxcounter}}%
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitlebackgroundcolor=red!10]{Philblock-pre}
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitle={Philosophical remarks},frametitlebackgroundcolor=red!10]{Philblock*}
\newenvironment{Philblock}[1][]{\begin{Philblock-pre}%
  [frametitle={Philosophical remarks \refstepcounter{philquestboxcounter}\setkeys{EPCPphilquest}{#1}\thephilquestboxcounter{} \EPCP@philquestTitle}%
  \renewcommand{\EPCP@philquestTitle}{}%
  ]}{\end{Philblock-pre}}%

% Experimental methods BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@expmethodsTitle}{}%
\define@key{EPCPexpmethod}{label}{\label{#1}}%
\define@key{EPCPexpmethod}{title}{\renewcommand{\EPCP@expmethodsTitle}{(\textsl{#1})}}%
\newcounter{expmethboxcounter}\setcounter{expmethboxcounter}{0}%
\renewcommand{\theexpmethboxcounter}{\arabic{chapter}.\arabic{section}.\alph{expmethboxcounter}}%
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitlebackgroundcolor=cyan!10]{Expblock-pre}
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitle={Experimental method},frametitlebackgroundcolor=cyan!10]{Expblock*}
\newenvironment{Expblock}[1][]{\begin{Expblock-pre}%
  [frametitle={Experimental method \refstepcounter{expmethboxcounter}\setkeys{EPCPexpmethod}{#1}\theexpmethboxcounter{} \EPCP@expmethodsTitle}%
  \renewcommand{\EPCP@expmethodsTitle}{}%
  ]}{\end{Expblock-pre}}%

\makeatother
% BOXES for other things %%%%%%%%%%%%%%%%%%%%%%%%%%%

\newmdenv[linecolor=black!50!black,
frametitlerule=true,
frametitle={},
frametitlebackgroundcolor=black!10%,
%frametitlefont={\sffamily\textcolor{white}}
]{Generalblock}

% Exercise environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{exercisecntr}
\setcounter{exercisecntr}{0}
\newenvironment{exercise}
  {%
   \par\noindent%
   \refstepcounter{exercisecntr}%
   \textbf{Exercise \theexercisecntr}}
  {\mbox{}}

==> ECPC book - Part V - UNC/backup_08_10_22/style-old.tex <==
\geometry{top=2cm,bottom=1.5cm,left=1.75cm,right=1.75cm}

\renewcommand*\familydefault{\sfdefault} %% Only if the base font of the document is to be sans serif

==> ECPC book - Part V - UNC/macros-chapter.tex <==
% This file contains a macro collection that can be used to (re-)define
% LaTeX macros when drafting a chapter.
%
% You can alter this source document but changes here will NOT be considered in the
% compiled book
%
\newcommand{\g}{\gamma}
\newcommand{\s}{\sigma}
\renewcommand{\L}{\Lambda}
\newcommand{\dkl}{D_{\text{KL}}}
\newcommand{\Wxi}{\mathcal{W}_{x_i}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\lp}{\log\!\text{-}\mathrm{cap}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\q}{\mathrm{q}}
\newcommand{\R}{\mathrm{r}}
\newcommand{\B}{\mathrm{b}}
\newcommand{\odds}{\mathrm{o}}
\newcommand{\diff}{\mathrm{d}}
\renewcommand{\underline}[1]{\mathbf{#1}}
\newcommand{\intsimpldetail}[2]{\int_{\mathbb{R}^M_+}\diff \mathbf{b} ~ \delta \left( \sum_{\tilde{x}} \B_{\tilde{x}} - #1 \right) ~ #2}
\newcommand{\intsimpl}[1]{\int_{\mathcal{B}} \diff \mathbf{b} ~ #1}
\newcommand{\N}{\noindent}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

==> ECPC book - Part V - UNC/main/macros-old.tex <==
% This is the central macro collection file that is used to define
% LaTeX macros for the final compiled book
%
% DO NOT APPLY ANY CHANGES TO THIS FILE UNLESS THIS WAS APPROVED BY THE BOOK EDITORS!
%
% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
%\usepackage[USenglish]{babel}
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{float}
\usepackage{geometry}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{lmodern}
\usepackage{mdframed}
\usepackage[numbers]{natbib}
\usepackage{siunitx}%
\usepackage{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MACROS ADDED on April 16th
%
% general %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[textsize=footnotesize,textwidth=2.8cm]{todonotes}
\usepackage[version=4]{mhchem}
%
% for chapter MET %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage[colorlinks=true, linkcolor=blue, urlcolor=blue]{hyperref}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\red[1]{\textcolor{red}{#1}}
%
% for chapter CBM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{physics}
\newcommand{\ve}[1]{\mathvectorfont{#1}}
\newcommand{\mat}[1]{\mathmatrixfont{#1}}
%
% for chapter SMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathtools}
%
% for chapter UNC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%
% for chapter PAT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Esc}{E}
\newcommand{\activity}{A}
\newcommand{\fluxcost}{a}
\newcommand{\hminus}{h}
\newcommand{\vPW}{v_{\rm pw}}
\newcommand{\enzymev}{\mathbf{e}}
\newcommand{\rrl}{\fluxcost_{v_l}}
\newcommand{\rrlmin}{\rrl^{\rm cat}}
\newcommand{\metbene}{b^{\rm (c)}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\concS}{s}
\newcommand{\concP}{p}
\newcommand{\e}{\mathrm{e}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\ratelaw}{f}
\definecolor{c1}{rgb}{0,0,0.8}
\definecolor{c2}{rgb}{0.25,0.,0.6}
\definecolor{c3}{rgb}{0.6,0.,0.3} 
\definecolor{c4}{rgb}{1,0,0}
\definecolor{c5}{rgb}{.5,0.2,0}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
% PROJECT SPECIFIC MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includechapterauthors}[1]{%
\par\noindent%
\textbf{Written by} #1\\[-3ex]%
}%

\newcommand{\chapteracknowledgments}[1]{
\par\noindent%
\textbf{Contributions:} #1\\[-3ex]%
}

\newcommand{\chapterkeywords}[1]{%
\par\noindent%
\textbf{Keywords:} #1\\[-3ex]%
}%

\newcommand{\comment}[1]{{\color{red}#1}}

\newcommand{\chapterroot}{./chapters/TEMPLATE/}% This refers to chapter directory

\newcommand{\copyrightinfo}[1]%{}
  {{\color{magenta}\textsc{Copyright Info:} #1}}

%
% Math macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Real}{\mathbb{R}} % real numbers
\newcommand{\Natu}{\mathbb{N}} % natural numbers
\newcommand{\Inte}{\mathbb{Z}} % integers
%
\newcommand{\expe}{\mathrm{e}}% Euler s number
\newcommand{\imagi}{\mathrm{i}}% imaginary unit
\newcommand{\intd}{\mathrm{d}}% differential-d
%
\newcommand{\mathvectorfont}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mathmatrixfont}[1]{\mathbf{#1}}
%
\newcommand{\avec}{\mathvectorfont{a}}
\newcommand{\varphivec}{\mathvectorfont{\varphi}}
%
\newcommand{\Amat}{\mathmatrixfont{A}}

%
% Metabolic modeling macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\kcat}{k_{\rm cat}}
\newcommand{\kcati}{k_{\rm cat,i}}
\newcommand{\kcatl}{k_{{\rm cat},l}}
\newcommand{\kcatplus}{k_{\rm cat}^+}
\newcommand{\kcatplusl}{k_{{\rm cat},l}^+}
\newcommand{\kcatminus}{k_{\rm cat}^-}
\newcommand{\km}{K_{{\rm M}}}
\newcommand{\kmS}{K_{{\rm S}}}
\newcommand{\kmP}{K_{{\rm P}}}
\newcommand{\Keq}{K_{\rm eq}} % equilibrium constant

% BOXES :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% To make use of
% (a) (future) key-value extensions,
% (b) numbering,
% (c) referencing and
% (d) mdframed boxes,
% we use the following "hack":
% (i) use mdframed for the definition of the boxes
% (ii) wrap them in "classically defined" environments that take care of labels, titles etc.
%
% MAYBE: - easier handling/cleaner code when using "startcode" and "endcode" from the mdframed package?
%  - "derive" everything from one "numbered box" code?
%  - change numbering (e.g. all boxes together)?
%
\makeatletter
% CHAPTER HIGHLIGHTS BOX %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newmdenv[linecolor=blue!50!black,
frametitlerule=true,
frametitle={Chapter highlights},
frametitlebackgroundcolor=blue!10%,
]{chapterhighlights}

% ECONOMIC ANALOGY BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@ecoanaTitle}{}%
\define@key{EPCPecoana}{label}{\label{#1}}%
\define@key{EPCPecoana}{title}{\renewcommand{\EPCP@ecoanaTitle}{(\textsl{#1})}}%
\newcounter{ecoanaboxcounter}\setcounter{ecoanaboxcounter}{0}%
\renewcommand{\theecoanaboxcounter}{\arabic{chapter}.\arabic{section}.\alph{ecoanaboxcounter}}%
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitlebackgroundcolor=blue!10]{Ecoblock-pre}
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitle={Economic analogy},frametitlebackgroundcolor=blue!10]{Ecoblock*}
\newenvironment{Ecoblock}[1][]{\begin{Ecoblock-pre}%
  [frametitle={Economic analogy \refstepcounter{ecoanaboxcounter}\setkeys{EPCPecoana}{#1}\theecoanaboxcounter{} \EPCP@ecoanaTitle}%
  \renewcommand{\EPCP@ecoanaTitle}{}%
  ]}{\end{Ecoblock-pre}}%

% Philosophcal question BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@philquestTitle}{}%
\define@key{EPCPphilquest}{label}{\label{#1}}%
\define@key{EPCPphilquest}{title}{\renewcommand{\EPCP@philquestTitle}{(\textsl{#1})}}%
\newcounter{philquestboxcounter}\setcounter{philquestboxcounter}{0}%
\renewcommand{\thephilquestboxcounter}{\arabic{chapter}.\arabic{section}.\alph{philquestboxcounter}}%
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitlebackgroundcolor=red!10]{Philblock-pre}
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitle={Philosophical remarks},frametitlebackgroundcolor=red!10]{Philblock*}
\newenvironment{Philblock}[1][]{\begin{Philblock-pre}%
  [frametitle={Philosophical remarks \refstepcounter{philquestboxcounter}\setkeys{EPCPphilquest}{#1}\thephilquestboxcounter{} \EPCP@philquestTitle}%
  \renewcommand{\EPCP@philquestTitle}{}%
  ]}{\end{Philblock-pre}}%

% Experimental methods BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@expmethodsTitle}{}%
\define@key{EPCPexpmethod}{label}{\label{#1}}%
\define@key{EPCPexpmethod}{title}{\renewcommand{\EPCP@expmethodsTitle}{(\textsl{#1})}}%
\newcounter{expmethboxcounter}\setcounter{expmethboxcounter}{0}%
\renewcommand{\theexpmethboxcounter}{\arabic{chapter}.\arabic{section}.\alph{expmethboxcounter}}%
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitlebackgroundcolor=cyan!10]{Expblock-pre}
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitle={Experimental method},frametitlebackgroundcolor=cyan!10]{Expblock*}
\newenvironment{Expblock}[1][]{\begin{Expblock-pre}%
  [frametitle={Experimental method \refstepcounter{expmethboxcounter}\setkeys{EPCPexpmethod}{#1}\theexpmethboxcounter{} \EPCP@expmethodsTitle}%
  \renewcommand{\EPCP@expmethodsTitle}{}%
  ]}{\end{Expblock-pre}}%

\makeatother
% BOXES for other things %%%%%%%%%%%%%%%%%%%%%%%%%%%

\newmdenv[linecolor=black!50!black,
frametitlerule=true,
frametitle={},
frametitlebackgroundcolor=black!10%,
%frametitlefont={\sffamily\textcolor{white}}
]{Generalblock}

% Exercise environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{exercisecntr}
\setcounter{exercisecntr}{0}
\newenvironment{exercise}
  {%
   \par\noindent%
   \refstepcounter{exercisecntr}%
   \textbf{Exercise \theexercisecntr}}
  {\mbox{}}

==> ECPC book - Part V - UNC/main/macros.tex <==
% This is the central macro collection file that is used to define
% LaTeX macros for the final compiled book
%
% DO NOT APPLY ANY CHANGES TO THIS FILE UNLESS THIS WAS APPROVED BY THE BOOK EDITORS!
%
% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
%\usepackage[USenglish]{babel}
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{float}
\usepackage{geometry}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{lmodern}
\usepackage{mdframed}
\usepackage[numbers]{natbib}
\usepackage{siunitx}%
\usepackage{xcolor}
\usepackage{pgfplots}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{setspace}
\usepackage{chngcntr}
\usepackage{enumitem}
%\pgfplotsset{compat=1.18}

\usepackage[nottoc,notlot,notlof]{tocbibind} % make sure bibliography appears in table of contents


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MACROS ADDED on April 16th
%
% general %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[textsize=footnotesize,textwidth=2.8cm]{todonotes}
\usepackage[version=4]{mhchem}
%
\ifx\tmpmacrosfolder\undefined% check if someone overwrote the location of tmp_macros.tex
  \newcommand{\tmpmacrosfolder}{.}%
\fi
\ifx\weAreInMain\undefined
{}
\else
\input{\tmpmacrosfolder/tmp_macros_chapters.tex}%
\fi
%
\usepackage[hidelinks]{hyperref}
% NOTE THAT THE USAGE OF HYPERREF SOMETIMES CAUSE TROUBLES
% if an old .aux file is present; to fix this, use cleantex and compile again
\definecolor{darkblue}{rgb}{0.15,0.,0.65}
\hypersetup{
	colorlinks=true,
	linkcolor=darkblue,
	filecolor=magenta,
        citecolor=darkblue,
	urlcolor=darkblue,
	pdftitle={Economic Principles in Cell Biology},
}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
% PROJECT SPECIFIC MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includechapterauthors}[1]{%
\par\noindent%
%\textbf{By}
#1\\%[-3ex]%
}%

\newcommand{\chapteracknowledgments}[1]{
\par\noindent%
\textbf{Contributions:} #1\\[-3ex]%
}

\newcommand{\chapterkeywords}[1]{%
\par\noindent%
\textbf{Keywords:} #1\\[-3ex]%
}%

\newcommand{\comment}[1]{{\color{red}#1}}

\newcommand{\chapterroot}{./chapters/TEMPLATE/}% This refers to chapter directory

\newcommand{\copyrightinfo}[1]%{}
  {{\color{magenta}\textsc{Copyright Info:} #1}}

%
% Math macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Real}{\mathbb{R}} % real numbers
\newcommand{\Natu}{\mathbb{N}} % natural numbers
\newcommand{\Inte}{\mathbb{Z}} % integers
%
\newcommand{\expe}{\mathrm{e}}% Euler s number
\newcommand{\imagi}{\mathrm{i}}% imaginary unit
\newcommand{\intd}{\mathrm{d}}% differential-d
%
\newcommand{\mathvectorfont}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mathmatrixfont}[1]{\mathbf{#1}}
%
\newcommand{\avec}{\mathvectorfont{a}}
\newcommand{\varphivec}{\mathvectorfont{\varphi}}
%
\newcommand{\Amat}{\mathmatrixfont{A}}
\newcommand{\Stoichmat}{\mathmatrixfont{N}}
%

% Macro for stuff that should only be shown in single-chapter layout

\newcommand{\hideinbooklayout}[1]{#1}

% BOXES :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% To make use of
% (a) (future) key-value extensions,
% (b) numbering,
% (c) referencing and
% (d) mdframed boxes,
% we use the following "hack":
% (i) use mdframed for the definition of the boxes
% (ii) wrap them in "classically defined" environments that take care of labels, titles etc.
% 
% MAYBE: - easier handling/cleaner code when using "startcode" and "endcode" from the mdframed package?
%  - change numbering (e.g. all boxes together)?
%
\floatstyle{plain}%
\newfloat{EPCPFloatBlock}{b}{loepcpb}[chapter]% "list of EPCP blocks"

\mdfdefinestyle{EPCPBlocks}{%
  linecolor=blue!50!black,%
  frametitlerule=true,%
  frametitlebackgroundcolor=\EPCPBlockTitleColor,%
  backgroundcolor=\EPCPBlockBGColor,%
  innertopmargin=9pt,% default: 5pt
  innerbottommargin=9pt,% default: 5pt
  skipabove=7pt,% default 0
  skipbelow=7pt%,% default 0
}
\newmdenv[style=EPCPBlocks]{EPCPBlockMD}%


\makeatletter
\newcommand{\EPCPBlockTitleFont}{\normalfont\bfseries}%
%\definecolor{EPCPviolet}{RGB}{102,0,255}
\definecolor{EPCPviolet}{rgb}{0.15,0.,0.65}
\newcommand{\EPCPBlockTitleFontColor}{EPCPviolet}
\newcommand{\EPCPBlockTitleColor}{EPCPviolet!10}
\newcommand{\EPCPBlockBGColor}{EPCPviolet!3}
% CHAPTER HIGHLIGHTS BOX %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newmdenv[style=EPCPBlocks,frametitle={\color{\EPCPBlockTitleFontColor}Chapter highlights}%
]{chapterhighlights}

% ECONOMIC ANALOGY BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@FloatSpec}{X}%
\newcommand{\EPCP@BlockTitle}{}%
%\define@key{EPCPecoana}{label}{\label{#1}}%
%\define@key{EPCPecoana}{title}{\renewcommand{\EPCP@BlockTitle}{:~{\EPCPBlockTitleFont#1}}}%
%\define@key{EPCPecoana}{float}{\renewcommand{\EPCP@FloatSpec}{#1}}%
\define@key{EPCPBlocks}{label}{\label{#1}}%
\define@key{EPCPBlocks}{title}{\renewcommand{\EPCP@BlockTitle}{:~{\EPCPBlockTitleFont#1}}}%
\define@key{EPCPBlocks}{float}{\renewcommand{\EPCP@FloatSpec}{#1}}%
\newcounter{ecoanaboxcounter}\setcounter{ecoanaboxcounter}{0}%
\newcounter{dummycounter}\setcounter{ecoanaboxcounter}{0}%
\counterwithin{ecoanaboxcounter}{chapter}% reset ecol. analogy box counter for each chapter
\renewcommand{\theecoanaboxcounter}{\arabic{chapter}.\Alph{ecoanaboxcounter}}% short box numbers
%
\newenvironment{EPCPBlock}[3][]%
{% begin env.
\setkeys{EPCPBlocks}{#1}%
\ifthenelse{\equal{\EPCP@FloatSpec}{X}}
{%Default
\begin{EPCPBlockMD}%
[frametitle={\color{\EPCPBlockTitleFontColor}#2#3\EPCP@BlockTitle}]
}
{%float version
\floatplacement{EPCPFloatBlock}{\EPCP@FloatSpec}%
\begin{EPCPFloatBlock}\begin{EPCPBlockMD}%
  [frametitle={\color{\EPCPBlockTitleFontColor}#2#3\EPCP@BlockTitle}]%
}%
}{% end env.
\ifthenelse{\equal{\EPCP@FloatSpec}{X}}
{%Default
\end{EPCPBlockMD}
}
{% float version
\end{EPCPBlockMD}\end{EPCPFloatBlock}
}
}% end EPCPblock

% Economic Analogy Block %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{Ecoblock}[1][]%
{\begin{EPCPBlock}[#1]{Economic analogy\mbox{~}}{\refstepcounter{ecoanaboxcounter}\theecoanaboxcounter}}
{\end{EPCPBlock}}
%
\newenvironment{Ecoblock*}[1][]%
{\begin{EPCPBlock}[#1]{Economic analogy}{}}
{\end{EPCPBlock}}
%

% Philosophical question BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{philquestboxcounter}\setcounter{philquestboxcounter}{0}%
\counterwithin{philquestboxcounter}{chapter}% reset phil. box counter for each chapter
\renewcommand{\thephilquestboxcounter}{\arabic{chapter}.\Alph{philquestboxcounter}}% short box numbers
\newenvironment{Philblock}[1][]%
{\begin{EPCPBlock}[#1]{Philosophical remarks\mbox{~}}{\refstepcounter{philquestboxcounter}\thephilquestboxcounter}}
{\end{EPCPBlock}}
%
\newenvironment{Philblock*}[1][]%
{\begin{EPCPBlock}[#1]{Philosophical remarks}{}}
{\end{EPCPBlock}}
%

% Experimental Methods Block %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{expmethboxcounter}\setcounter{expmethboxcounter}{0}%
\counterwithin{expmethboxcounter}{chapter}% reset exp-meth. box counter for each chapter
\renewcommand{\theexpmethboxcounter}{\arabic{chapter}.\Alph{expmethboxcounter}}% short box numbers
\newenvironment{Expblock}[1][]%
{\begin{EPCPBlock}[#1]{Experimental methods\mbox{~}}{\refstepcounter{expmethboxcounter}\theexpmethboxcounter}}
{\end{EPCPBlock}}
%
\newenvironment{Expblock*}[1][]%
{\begin{EPCPBlock}[#1]{Experimental methods}{}}
{\end{EPCPBlock}}
%

% Mathematical Details BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{mathdetailboxcounter}\setcounter{mathdetailboxcounter}{0}%
\counterwithin{mathdetailboxcounter}{chapter}% reset math box counter for each chapter
\renewcommand{\themathdetailboxcounter}{\arabic{chapter}.\Alph{mathdetailboxcounter}}%
\newenvironment{MathDetailblock}[1][]%
{\begin{EPCPBlock}[#1]{Mathematical details\mbox{~}}{\refstepcounter{mathdetailboxcounter}\themathdetailboxcounter}}
{\end{EPCPBlock}}
%
\newenvironment{MathDetailblock*}[1][]%
{\begin{EPCPBlock}[#1]{Mathematical details}{}}
{\end{EPCPBlock}}

% GENERAL BOXES for other things %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@GeneralBlockTitle}{A}%
\define@key{EPCPGeneralblock}{title}{\renewcommand{\EPCP@GeneralBlockTitle}{{\EPCPBlockTitleFont#1}}}%
\newenvironment{Generalblock}[1][]{\setkeys{EPCPGeneralblock}{#1}%
\ifthenelse{\equal{\EPCP@GeneralBlockTitle}{A}}%
{\begin{EPCPBlockMD}}%
%\else%
{\begin{EPCPBlockMD}[frametitle={\color{\EPCPBlockTitleFontColor}\EPCP@GeneralBlockTitle}]}%
%\fi%
}{\end{EPCPBlockMD}%
\renewcommand{\EPCP@GeneralBlockTitle}{A}}
\makeatother

% Exercise environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{exercisecntr}
\setcounter{exercisecntr}{0}
\counterwithin{exercisecntr}{chapter}% reset exercise counter for each chapter
\newenvironment{exercise}
  {%
   \par\noindent%
   \refstepcounter{exercisecntr}%
   \textbf{Exercise \theexercisecntr}}
  {\mbox{}}


==> ECPC book - Part V - UNC/main/style.tex <==
\geometry{top=2cm,bottom=2cm,left=1.75cm,right=1.75cm}

\renewcommand*\familydefault{\sfdefault} %% Only if the base font of the document is to be sans serif

\setlength{\parindent}{0pt}
\setlength{\parskip}{2mm}

% https://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html
\setlength{\floatsep}{5pt plus 5pt}%
\setlength{\abovecaptionskip}{5pt plus 5pt}%
\setlength{\belowcaptionskip}{5pt plus 5pt}%
%\floatsep: space left between floats.
%\textfloatsep: space between last top float or first bottom float and the text.
%\intextsep : space left on top and bottom of an in-text float.
%\dbltextfloatsep is \textfloatsep for 2 column output.
%\dblfloatsep is \floatsep for 2 column output.
%\abovecaptionskip: space above caption
%\belowcaptionskip: space below caption
\renewcommand\floatpagefraction{.9}
\renewcommand\dblfloatpagefraction{.9} % for two column documents
\renewcommand\topfraction{.9}

==> ECPC book - Part V - UNC/style-chapter.tex <==
% This file contains local style definition file that can be used to (re-)define
% the look-and-feel when drafting a chapter.
%
% You can alter this source document but changes here will NOT be considered in the
% compiled book.
% 
\usepackage{setspace}
\usepackage[final
           ]{showkeys}% removing the "final" option displays labels and citations.
%
\definecolor{refkey}{rgb}{.65,.65,.65}
\definecolor{labelkey}{rgb}{.65,.65,.65}
\renewcommand*\showkeyslabelformat[1]{%
    \fbox{\resizebox{1.75cm}{!}{\normalfont\ttfamily#1}}}
%
% If you do not like the sans serif of the main document
\renewcommand*\familydefault{\rmdefault} 


% 1.5-spacing and wider margins for easier drafting/reviewing
\onehalfspacing
\geometry{right=3cm,left=3cm,marginparwidth=2.8cm}

% make list environments "tighter"
\usepackage{enumitem}
\setlist{noitemsep}


==> backup_08_10_22/macros-old.tex <==
% This is the central macro collection file that is used to define
% LaTeX macros for the final compiled book
%
% DO NOT APPLY ANY CHANGES TO THIS FILE UNLESS THIS WAS APPROVED BY THE BOOK EDITORS!
%
% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
%\usepackage[USenglish]{babel}
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{float}
\usepackage{geometry}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{lmodern}
\usepackage{mdframed}
\usepackage[numbers]{natbib}
\usepackage{siunitx}%
\usepackage{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MACROS ADDED on April 16th
%
% general %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[textsize=footnotesize,textwidth=2.8cm]{todonotes}
\usepackage[version=4]{mhchem}
%
% for chapter MET %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage[colorlinks=true, linkcolor=blue, urlcolor=blue]{hyperref}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\red[1]{\textcolor{red}{#1}}
%
% for chapter CBM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{physics}
\newcommand{\ve}[1]{\mathvectorfont{#1}}
\newcommand{\mat}[1]{\mathmatrixfont{#1}}
%
% for chapter SMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathtools}
%
% for chapter UNC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\s}{\sigma}
\renewcommand{\L}{\Lambda}
\newcommand{\dkl}{D_{\text{KL}}}
\newcommand{\Wxi}{\mathcal{W}_{x_i}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\lp}{\log\!\text{-}\mathrm{cap}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\R}{\mathrm{r}}
\newcommand{\B}{\mathrm{b}}
\newcommand{\odds}{\mathrm{o}}
\newcommand{\diff}{\mathrm{d}}
\renewcommand{\underline}[1]{\mathbf{#1}}
\newcommand{\intsimpldetail}[2]{\int_{\mathbb{R}^M_+}\diff \mathbf{b} ~ \delta \left( \sum_{\tilde{x}} \B_{\tilde{x}} - #1 \right) ~ #2}
\newcommand{\intsimpl}[1]{\int_{\mathcal{B}} \diff \mathbf{b} ~ #1}
\newcommand{\N}{\noindent}
%
%
% for chapter PAT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Esc}{E}
\newcommand{\activity}{A}
\newcommand{\fluxcost}{a}
\newcommand{\hminus}{h}
\newcommand{\vPW}{v_{\rm pw}}
\newcommand{\enzymev}{\mathbf{e}}
\newcommand{\rrl}{\fluxcost_{v_l}}
\newcommand{\rrlmin}{\rrl^{\rm cat}}
\newcommand{\metbene}{b^{\rm (c)}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\concS}{s}
\newcommand{\concP}{p}
\newcommand{\e}{\mathrm{e}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\ratelaw}{f}
\definecolor{c1}{rgb}{0,0,0.8}
\definecolor{c2}{rgb}{0.25,0.,0.6}
\definecolor{c3}{rgb}{0.6,0.,0.3} 
\definecolor{c4}{rgb}{1,0,0}
\definecolor{c5}{rgb}{.5,0.2,0}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
% PROJECT SPECIFIC MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includechapterauthors}[1]{%
\par\noindent%
\textbf{Written by} #1\\[-3ex]%
}%

\newcommand{\chapteracknowledgments}[1]{
\par\noindent%
\textbf{Contributions:} #1\\[-3ex]%
}

\newcommand{\chapterkeywords}[1]{%
\par\noindent%
\textbf{Keywords:} #1\\[-3ex]%
}%

\newcommand{\comment}[1]{{\color{red}#1}}

\newcommand{\chapterroot}{./chapters/TEMPLATE/}% This refers to chapter directory

\newcommand{\copyrightinfo}[1]%{}
  {{\color{magenta}\textsc{Copyright Info:} #1}}

%
% Math macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Real}{\mathbb{R}} % real numbers
\newcommand{\Natu}{\mathbb{N}} % natural numbers
\newcommand{\Inte}{\mathbb{Z}} % integers
%
\newcommand{\expe}{\mathrm{e}}% Euler s number
\newcommand{\imagi}{\mathrm{i}}% imaginary unit
\newcommand{\intd}{\mathrm{d}}% differential-d
%
\newcommand{\mathvectorfont}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mathmatrixfont}[1]{\mathbf{#1}}
%
\newcommand{\avec}{\mathvectorfont{a}}
\newcommand{\varphivec}{\mathvectorfont{\varphi}}
%
\newcommand{\Amat}{\mathmatrixfont{A}}

%
% Metabolic modeling macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\kcat}{k_{\rm cat}}
\newcommand{\kcati}{k_{\rm cat,i}}
\newcommand{\kcatl}{k_{{\rm cat},l}}
\newcommand{\kcatplus}{k_{\rm cat}^+}
\newcommand{\kcatplusl}{k_{{\rm cat},l}^+}
\newcommand{\kcatminus}{k_{\rm cat}^-}
\newcommand{\km}{K_{{\rm M}}}
\newcommand{\kmS}{K_{{\rm S}}}
\newcommand{\kmP}{K_{{\rm P}}}
\newcommand{\Keq}{K_{\rm eq}} % equilibrium constant

% BOXES :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% To make use of
% (a) (future) key-value extensions,
% (b) numbering,
% (c) referencing and
% (d) mdframed boxes,
% we use the following "hack":
% (i) use mdframed for the definition of the boxes
% (ii) wrap them in "classically defined" environments that take care of labels, titles etc.
%
% MAYBE: - easier handling/cleaner code when using "startcode" and "endcode" from the mdframed package?
%  - "derive" everything from one "numbered box" code?
%  - change numbering (e.g. all boxes together)?
%
\makeatletter
% CHAPTER HIGHLIGHTS BOX %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newmdenv[linecolor=blue!50!black,
frametitlerule=true,
frametitle={Chapter highlights},
frametitlebackgroundcolor=blue!10%,
]{chapterhighlights}

% ECONOMIC ANALOGY BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@ecoanaTitle}{}%
\define@key{EPCPecoana}{label}{\label{#1}}%
\define@key{EPCPecoana}{title}{\renewcommand{\EPCP@ecoanaTitle}{(\textsl{#1})}}%
\newcounter{ecoanaboxcounter}\setcounter{ecoanaboxcounter}{0}%
\renewcommand{\theecoanaboxcounter}{\arabic{chapter}.\arabic{section}.\alph{ecoanaboxcounter}}%
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitlebackgroundcolor=blue!10]{Ecoblock-pre}
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitle={Economic analogy},frametitlebackgroundcolor=blue!10]{Ecoblock*}
\newenvironment{Ecoblock}[1][]{\begin{Ecoblock-pre}%
  [frametitle={Economic analogy \refstepcounter{ecoanaboxcounter}\setkeys{EPCPecoana}{#1}\theecoanaboxcounter{} \EPCP@ecoanaTitle}%
  \renewcommand{\EPCP@ecoanaTitle}{}%
  ]}{\end{Ecoblock-pre}}%

% Philosophcal question BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@philquestTitle}{}%
\define@key{EPCPphilquest}{label}{\label{#1}}%
\define@key{EPCPphilquest}{title}{\renewcommand{\EPCP@philquestTitle}{(\textsl{#1})}}%
\newcounter{philquestboxcounter}\setcounter{philquestboxcounter}{0}%
\renewcommand{\thephilquestboxcounter}{\arabic{chapter}.\arabic{section}.\alph{philquestboxcounter}}%
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitlebackgroundcolor=red!10]{Philblock-pre}
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitle={Philosophical remarks},frametitlebackgroundcolor=red!10]{Philblock*}
\newenvironment{Philblock}[1][]{\begin{Philblock-pre}%
  [frametitle={Philosophical remarks \refstepcounter{philquestboxcounter}\setkeys{EPCPphilquest}{#1}\thephilquestboxcounter{} \EPCP@philquestTitle}%
  \renewcommand{\EPCP@philquestTitle}{}%
  ]}{\end{Philblock-pre}}%

% Experimental methods BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@expmethodsTitle}{}%
\define@key{EPCPexpmethod}{label}{\label{#1}}%
\define@key{EPCPexpmethod}{title}{\renewcommand{\EPCP@expmethodsTitle}{(\textsl{#1})}}%
\newcounter{expmethboxcounter}\setcounter{expmethboxcounter}{0}%
\renewcommand{\theexpmethboxcounter}{\arabic{chapter}.\arabic{section}.\alph{expmethboxcounter}}%
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitlebackgroundcolor=cyan!10]{Expblock-pre}
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitle={Experimental method},frametitlebackgroundcolor=cyan!10]{Expblock*}
\newenvironment{Expblock}[1][]{\begin{Expblock-pre}%
  [frametitle={Experimental method \refstepcounter{expmethboxcounter}\setkeys{EPCPexpmethod}{#1}\theexpmethboxcounter{} \EPCP@expmethodsTitle}%
  \renewcommand{\EPCP@expmethodsTitle}{}%
  ]}{\end{Expblock-pre}}%

\makeatother
% BOXES for other things %%%%%%%%%%%%%%%%%%%%%%%%%%%

\newmdenv[linecolor=black!50!black,
frametitlerule=true,
frametitle={},
frametitlebackgroundcolor=black!10%,
%frametitlefont={\sffamily\textcolor{white}}
]{Generalblock}

% Exercise environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{exercisecntr}
\setcounter{exercisecntr}{0}
\newenvironment{exercise}
  {%
   \par\noindent%
   \refstepcounter{exercisecntr}%
   \textbf{Exercise \theexercisecntr}}
  {\mbox{}}

==> backup_08_10_22/style-old.tex <==
\geometry{top=2cm,bottom=1.5cm,left=1.75cm,right=1.75cm}

\renewcommand*\familydefault{\sfdefault} %% Only if the base font of the document is to be sans serif

==> main/macros-old.tex <==
% This is the central macro collection file that is used to define
% LaTeX macros for the final compiled book
%
% DO NOT APPLY ANY CHANGES TO THIS FILE UNLESS THIS WAS APPROVED BY THE BOOK EDITORS!
%
% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
%\usepackage[USenglish]{babel}
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{float}
\usepackage{geometry}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{lmodern}
\usepackage{mdframed}
\usepackage[numbers]{natbib}
\usepackage{siunitx}%
\usepackage{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% MACROS ADDED on April 16th
%
% general %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[textsize=footnotesize,textwidth=2.8cm]{todonotes}
\usepackage[version=4]{mhchem}
%
% for chapter MET %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage[colorlinks=true, linkcolor=blue, urlcolor=blue]{hyperref}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\red[1]{\textcolor{red}{#1}}
%
% for chapter CBM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{physics}
\newcommand{\ve}[1]{\mathvectorfont{#1}}
\newcommand{\mat}[1]{\mathmatrixfont{#1}}
%
% for chapter SMA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathtools}
%
% for chapter UNC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%
% for chapter PAT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Esc}{E}
\newcommand{\activity}{A}
\newcommand{\fluxcost}{a}
\newcommand{\hminus}{h}
\newcommand{\vPW}{v_{\rm pw}}
\newcommand{\enzymev}{\mathbf{e}}
\newcommand{\rrl}{\fluxcost_{v_l}}
\newcommand{\rrlmin}{\rrl^{\rm cat}}
\newcommand{\metbene}{b^{\rm (c)}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\concS}{s}
\newcommand{\concP}{p}
\newcommand{\e}{\mathrm{e}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\ratelaw}{f}
\definecolor{c1}{rgb}{0,0,0.8}
\definecolor{c2}{rgb}{0.25,0.,0.6}
\definecolor{c3}{rgb}{0.6,0.,0.3} 
\definecolor{c4}{rgb}{1,0,0}
\definecolor{c5}{rgb}{.5,0.2,0}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
% PROJECT SPECIFIC MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includechapterauthors}[1]{%
\par\noindent%
\textbf{Written by} #1\\[-3ex]%
}%

\newcommand{\chapteracknowledgments}[1]{
\par\noindent%
\textbf{Contributions:} #1\\[-3ex]%
}

\newcommand{\chapterkeywords}[1]{%
\par\noindent%
\textbf{Keywords:} #1\\[-3ex]%
}%

\newcommand{\comment}[1]{{\color{red}#1}}

\newcommand{\chapterroot}{./chapters/TEMPLATE/}% This refers to chapter directory

\newcommand{\copyrightinfo}[1]%{}
  {{\color{magenta}\textsc{Copyright Info:} #1}}

%
% Math macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Real}{\mathbb{R}} % real numbers
\newcommand{\Natu}{\mathbb{N}} % natural numbers
\newcommand{\Inte}{\mathbb{Z}} % integers
%
\newcommand{\expe}{\mathrm{e}}% Euler s number
\newcommand{\imagi}{\mathrm{i}}% imaginary unit
\newcommand{\intd}{\mathrm{d}}% differential-d
%
\newcommand{\mathvectorfont}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mathmatrixfont}[1]{\mathbf{#1}}
%
\newcommand{\avec}{\mathvectorfont{a}}
\newcommand{\varphivec}{\mathvectorfont{\varphi}}
%
\newcommand{\Amat}{\mathmatrixfont{A}}

%
% Metabolic modeling macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\kcat}{k_{\rm cat}}
\newcommand{\kcati}{k_{\rm cat,i}}
\newcommand{\kcatl}{k_{{\rm cat},l}}
\newcommand{\kcatplus}{k_{\rm cat}^+}
\newcommand{\kcatplusl}{k_{{\rm cat},l}^+}
\newcommand{\kcatminus}{k_{\rm cat}^-}
\newcommand{\km}{K_{{\rm M}}}
\newcommand{\kmS}{K_{{\rm S}}}
\newcommand{\kmP}{K_{{\rm P}}}
\newcommand{\Keq}{K_{\rm eq}} % equilibrium constant

% BOXES :::::::::::::::::::::::::::::::::::::::::::::::::::::::
% To make use of
% (a) (future) key-value extensions,
% (b) numbering,
% (c) referencing and
% (d) mdframed boxes,
% we use the following "hack":
% (i) use mdframed for the definition of the boxes
% (ii) wrap them in "classically defined" environments that take care of labels, titles etc.
%
% MAYBE: - easier handling/cleaner code when using "startcode" and "endcode" from the mdframed package?
%  - "derive" everything from one "numbered box" code?
%  - change numbering (e.g. all boxes together)?
%
\makeatletter
% CHAPTER HIGHLIGHTS BOX %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newmdenv[linecolor=blue!50!black,
frametitlerule=true,
frametitle={Chapter highlights},
frametitlebackgroundcolor=blue!10%,
]{chapterhighlights}

% ECONOMIC ANALOGY BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@ecoanaTitle}{}%
\define@key{EPCPecoana}{label}{\label{#1}}%
\define@key{EPCPecoana}{title}{\renewcommand{\EPCP@ecoanaTitle}{(\textsl{#1})}}%
\newcounter{ecoanaboxcounter}\setcounter{ecoanaboxcounter}{0}%
\renewcommand{\theecoanaboxcounter}{\arabic{chapter}.\arabic{section}.\alph{ecoanaboxcounter}}%
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitlebackgroundcolor=blue!10]{Ecoblock-pre}
\newmdenv[linecolor=blue!50!black,frametitlerule=true,frametitle={Economic analogy},frametitlebackgroundcolor=blue!10]{Ecoblock*}
\newenvironment{Ecoblock}[1][]{\begin{Ecoblock-pre}%
  [frametitle={Economic analogy \refstepcounter{ecoanaboxcounter}\setkeys{EPCPecoana}{#1}\theecoanaboxcounter{} \EPCP@ecoanaTitle}%
  \renewcommand{\EPCP@ecoanaTitle}{}%
  ]}{\end{Ecoblock-pre}}%

% Philosophcal question BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@philquestTitle}{}%
\define@key{EPCPphilquest}{label}{\label{#1}}%
\define@key{EPCPphilquest}{title}{\renewcommand{\EPCP@philquestTitle}{(\textsl{#1})}}%
\newcounter{philquestboxcounter}\setcounter{philquestboxcounter}{0}%
\renewcommand{\thephilquestboxcounter}{\arabic{chapter}.\arabic{section}.\alph{philquestboxcounter}}%
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitlebackgroundcolor=red!10]{Philblock-pre}
\newmdenv[linecolor=red!50!black,frametitlerule=true,frametitle={Philosophical remarks},frametitlebackgroundcolor=red!10]{Philblock*}
\newenvironment{Philblock}[1][]{\begin{Philblock-pre}%
  [frametitle={Philosophical remarks \refstepcounter{philquestboxcounter}\setkeys{EPCPphilquest}{#1}\thephilquestboxcounter{} \EPCP@philquestTitle}%
  \renewcommand{\EPCP@philquestTitle}{}%
  ]}{\end{Philblock-pre}}%

% Experimental methods BOXES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EPCP@expmethodsTitle}{}%
\define@key{EPCPexpmethod}{label}{\label{#1}}%
\define@key{EPCPexpmethod}{title}{\renewcommand{\EPCP@expmethodsTitle}{(\textsl{#1})}}%
\newcounter{expmethboxcounter}\setcounter{expmethboxcounter}{0}%
\renewcommand{\theexpmethboxcounter}{\arabic{chapter}.\arabic{section}.\alph{expmethboxcounter}}%
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitlebackgroundcolor=cyan!10]{Expblock-pre}
\newmdenv[linecolor=cyan!50!black,frametitlerule=true,frametitle={Experimental method},frametitlebackgroundcolor=cyan!10]{Expblock*}
\newenvironment{Expblock}[1][]{\begin{Expblock-pre}%
  [frametitle={Experimental method \refstepcounter{expmethboxcounter}\setkeys{EPCPexpmethod}{#1}\theexpmethboxcounter{} \EPCP@expmethodsTitle}%
  \renewcommand{\EPCP@expmethodsTitle}{}%
  ]}{\end{Expblock-pre}}%

\makeatother
% BOXES for other things %%%%%%%%%%%%%%%%%%%%%%%%%%%

\newmdenv[linecolor=black!50!black,
frametitlerule=true,
frametitle={},
frametitlebackgroundcolor=black!10%,
%frametitlefont={\sffamily\textcolor{white}}
]{Generalblock}

% Exercise environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{exercisecntr}
\setcounter{exercisecntr}{0}
\newenvironment{exercise}
  {%
   \par\noindent%
   \refstepcounter{exercisecntr}%
   \textbf{Exercise \theexercisecntr}}
  {\mbox{}}
